Boosting in Image Quality Assessment

In this paper, we analyze the effect of boosting in image quality assessment through multi-method fusion. Existing multi-method studies focus on proposing a single quality estimator. On the contrary, we investigate the generalizability of multi-method fusion as a framework. In addition to support vector machines that are commonly used in the multi-method fusion, we propose using neural networks in the boosting. To span different types of image quality assessment algorithms, we use quality estimators based on fidelity, perceptually-extended fidelity, structural similarity, spectral similarity, color, and learning. In the experiments, we perform k-fold cross validation using the LIVE, the multiply distorted LIVE, and the TID 2013 databases and the performance of image quality assessment algorithms are measured via accuracy-, linearity-, and ranking-based metrics. Based on the experiments, we show that boosting methods generally improve the performance of image quality assessment and the level of improvement depends on the type of the boosting algorithm. Our experimental results also indicate that boosting the worst performing quality estimator with two or more additional methods leads to statistically significant performance enhancements independent of the boosting technique and neural network-based boosting outperforms support vector machine-based boosting when two or more methods are fused.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> sec_intro.tex <==
\section{Introduction}
\label{sec:intro}
\IEEEPARstart{E}very d



 
 
  
  
  
  .









==> sec_main.tex <==
\section{Preprocessing}
\label{sec:preprocess}
The main stages in the preprocessing pipeline are shown in Fig. \ref{fig:pre}. An input image is transformed from the RGB color domain to the YCbCr, and Y, Cr and G channels are fed to a patch sampling block. A reshaping block is used to vectorize the sampled patches. Mean values are subtracted from the vectorized patches, which are processed with a ZCA whitening block to obtain the output of the preprocessing stage.   

\begin{figure}[htbp!]
\begin{center}
\noindent
  \includegraphics[width=\linewidth]{Figs/pipeline_pre.PNG}
  \caption{Preprocessing pipeline.}
  \label{fig:pre}
\end{center}
\end{figure}
\subsection{Color Space Selection}
In addition to the green channel in the RGB color domain, the Y (luma) and the Cr channels are also used by the method in \cite{UNIQUE}. The luma channel is selected because the human visual system is more sensitive to changes in intensity compared to color \cite{lamb2001}. The R, the G, and the B channels are not used together because of the high correlation among them and the only selected channel out of an RGB image is the G, which contains most of the information already contained in the R and B channels \cite{tkalcic2003colour}. Cr is also used in \cite{UNIQUE} becaouse of the promising results in the experimentation.

\subsection{Patch-based sampling and reshaping}
An $8$ by $8$ patch is randomly sampled from a YGCr image and vectorized into a one dimensional representation of length $192$. The same operation is repeated $100$ times for each image.


\subsection{Mean subtraction and ZCA whitening}
The vectorized representation is decorrelated via ZCA whitening, which is based on whitening operations of retina and lateral geniculate nucelus in human visual system \cite{chang2012}.



\section{Sparse Representation}
\label{sec:decoder}

\subsection{Training set}
As in \cite{UNIQUE}, we use ImageNet database, which can contain the queried object along with other objects, multiple instances, occlusion or text \cite{fei13}. In the training phase, $1,000$ images are randomly selected and $100$ patches are obtained from each image.

\subsection{Sparse Representation Generation}
Sparse representaitons are obtained with a linear decoder, which is an unsupervised learning architecture used to represent the input data in different dimensions. The output of a linear decoder ($\hat{p}$) is the reconstructed version of the input ($p$), which is used in the backpropogation stage to adjust the weight $W$ and bias $b$ as shown in Fig. \ref{fig:decoder}. 
\begin{figure}[htbp!]
	\begin{center}
		\noindent
		\includegraphics[width=0.6\linewidth]{Figs/pipeline_decoder.PNG}
		\caption{Linear decoder architecture, where NL is the non-linear sigmoid layer.}
		\label{fig:decoder}
		\vspace{-5.0mm}
	\end{center}
\end{figure}
The input representation is transformed into a different dimension with the weight $W_1$ and a bias ($b_1$) is added. Then, it is passed through a non-linear sigmoid activation function ($NL$).  The objective function $J(W_1,W_2,b_1,b_2)$ is minimized using the backpropogation operation.
$W_2$ and $b_2$ are the reconstruction weights and bias. Adding a sparsity constraint $\rho$, the objective function to be minimized can be expressed as 
\begin{equation}\label{LinearDecoder}
	J(W_1,W_2,b_1,b_2) = \lVert (W_2's + b_2) - P \rVert_2^2 + \rho \lVert s \rVert_1,
\end{equation}
where the first term is the reconstruction error while the second term is the sparsity constraint. Note that $s$ is a function of $W_1$ and $b_1$ as in (\ref{AutoSparse}) and hence minimization is performed over weights and bias in both encoding and decoding stages using L-BFGS algorithm. $\rho$ is set to $0.035$ to limit the average activation of neurons. As shown in Fig. \ref{fig:decoder},  an image patch of size $192$x$1$ is mapped to a sparse representation of size $400$x$1$.  



\section{Sparse Coding}
\label{sec:coding}
After we derive the weights and bias that provide us the structure and color encompassing transformation, we turn to compactly representing all such transformed patches in the form of a sparse codebook. The goal of sparse coding is to learn an over-complete set of basis vectors $\phi_i$ so that we can represent any transformed patch $s_i$ as a linear combination such basis vectors.
\begin{equation}
s = \sum_{i=1}^{N} a_i \phi_i
\end{equation}

where $s$ is the sparse representation of patches $p$ and $a$ are the non-unique sparse coefficients. To resolve degeneracy due to over-completeness, we optimize using a sparsity penalty $\lambda_{SC}$. Since both $a$ and $\phi$ are assigned randomly in the beginning, we minimize for
\begin{equation}
J_{SC}(A,\phi) = \lVert A\phi - s \rVert_2^2 + \lambda \lVert s \rVert_1 + \gamma\lVert A \rVert_2^2
\end{equation}
where $\gamma$ is a weight decay parameter designed to limit values in $A$.
Note that this equation is very similar to eq.\ref{LinearDecoder}. Hence, we use an autoencoder framework for minimization. However, the objective function is not differentiable at $0$ which is a requirement for using gradient based optimization methods which are used in autoencoders. This is achieved by smoothing out the L1 norm of $s$ using $\epsilon$ as a smoothing parameter. The updated objective function is 
\begin{equation} \label{SparseCoding}
J_{SC}(A,\phi) = \lVert A\phi - s \rVert_2^2 + \lambda \sqrt{\phi^2 + \epsilon} + \gamma\lVert A \rVert_2^2
\end{equation}

\subsection{Training Set}
To validate our sparse representation and prevent overfitting in our codebook, we again choose another set of random 100000 patches from the same database, transform them and build the codebook from them. During the said transformation, the same preprocessing steps as outlined before are followed to get $192x100000$ patches. On the preprocessed patches, the weights and bias learnt from the previous section are applied along with a non linear sigmoid layer at the end. We end up with a transformed $400x100000$ matrix.

\subsection{Batching and number of codewords}
Since in eq.\ref{SparseCoding} we minimize for both $A$ and $\phi$, the iteration process for a full batch of 100000 patches is time inhibitive. In order to avoid such a scenario, we divide it into mini batches of $N$ patches which are randomly selected in each iteration. At the end of training phase we will be left with $\phi$, a $400xN$ matrix. Hence, $N$ determines the number of codewords generated.

\subsection{Initialization of $A$ and $\phi$} \label{Initializing}
The objective function in eq.\ref{SparseCoding} is non-convex. However, solving for $\phi$ given $A$ in $J_{SC}(A,\phi)$ is convex and similarly solving for $A$ given $\phi$ is convex. Hence, we employ an alternative dual minimization strategy to solve for the non-convex objective function. While doing so, we randomly initialize $A$. For setting $\phi$, we follow the following steps :
\begin{itemize}
	\item $\phi_{initial}$ = $A^{T}s$. This is intuitive since we ideally need $s = A\phi_{initial}$.
	\item Each codeword in $\phi$ is normalized using the corresponding columns of sparse coefficients in $A$. Therefore, $\phi_i = \dfrac{\phi_{initial}}{\lVert A_i \rVert_1}$. Doing so reduces $\phi$ values which keeps the sparsity penalty small.
\end{itemize}
Also, the rate of convergence is increased by following the above initialization steps.
\subsection{Topographic sparse coding}
Sparse coding draws inspiration from the brain in simulating edge detection in the V1 cortex area. Topographic sparse coding is an extension of this inspiration by assuming that adjacent neurons detect edges at similar orientations. This has been extensively explored in literature \cite{Hyvärinen20012413}\cite{hyvarinen2001topographic}\cite{5206545}. 
Using a grouping matrix $V$ as described in \cite{UFLDL} we update the minimization function in Eq.\ref{SparseCoding} as
\begin{equation} \label{FinalSparseCoding}
J_{SC}(A,\phi) = \lVert A\phi - s \rVert_2^2 + \lambda \sqrt{V\phi\phi^T + \epsilon} + \gamma\lVert A \rVert_2^2
\end{equation}
\subsection{Codebook Generation}
The procedure to generate codebook is outlined below.
\begin{algorithm}[H]
	\caption{\label{alg:CodebookGeneration}Codebook Generation}
	\textbf{\footnotesize Iterative steps}{\footnotesize \par}
	\begin{enumerate}
		\item {\footnotesize Randomly select a mini batch of transformed patches of size $N = 10000$ from the complete batch of $100000$ transformed patches}{\footnotesize \par}
		\item {\footnotesize Initialize $A$ randomly.}{\footnotesize \par}
		\item {\footnotesize Initialize $\phi$ as described in Section \ref{Initializing} }{\footnotesize \par}
		\item {\footnotesize Assuming $A$ to be correct, find $\phi'$ that minimizes $J_{SC}(A,\phi)$ from eq.\ref{FinalSparseCoding} {\footnotesize \par}}
		\item {\footnotesize Solve for $A$ that minimizes  $J_{SC}(A,\phi')$ to obtain $A'$ {\footnotesize \par}}
		\item {\footnotesize Repeat until convergence {\footnotesize \par}}
	\end{enumerate}
\end{algorithm}
A single iteration of the process is shown as a block diagram in fig \ref{fig:Iteration}.
\begin{figure}[htbp!]
	\begin{center}
		\noindent
		\includegraphics[width=\linewidth]{Figs/SparseCodebook.PNG}
		\caption{Updating sparse coefficients and codebook}
		\label{fig:Iteration}
	\end{center}
\end{figure}

\begin{figure}[htbp!]
	\begin{center}
		\noindent
		\includegraphics[width=\linewidth]{Figs/Codebook.PNG}
		\caption{Visualization of learned features.}
		\label{fig:CodebookVis}
	\end{center}
\end{figure}

\section{Image quality estimation}
\label{sec:est}
Image quality estimation pipeline is shown in Fig. \ref{fig:main}. Training is performed in an unsupervised fashion by feeding preprocessed patches into a linear decoder. The learned weights and bias are used to transform preprocessed non-overlapping patches of the reference and compared image into sparse representations. If an entity in the sparse representation is significantly less than the average activation value, a zero is assigned to mimic the suppression mechanisms in the visual system. Spearman rank order correlation coefficient is used to compare the two reshaped vectors and we use  $10^{th}$ power of the correlation coefficient to utilize the full quality estiamte range.

\begin{figure}[htbp!]
	\begin{center}
		\noindent
		\includegraphics[width=\linewidth]{Figs/pipeline_main.PNG}
		\caption{Image quality estimation pipeline.}
		\label{fig:main}
	\end{center}
\end{figure}




==> sec_validation.tex <==
\section{Validation}
\label{sec:val}





\subsection{Databases}



In the comparison of the quality estimators, we use the LIVE image quality database \cite{live2006}, multiply distorted LIVE (MULTI) database \cite{multi2012} and TID 2013 (TID13) database \cite{tid13}. The distortion types in these databases can be classified into seven groups. Compression group consists of JPEG compression, JPEG2000 compression and lossy compression of noisy images. Noise group includes additive Gaussian noise, additive noise in color components which is more intensive than additive noise in the luminance component, spatially correlated noise, masked noise, high frequency noise, impulse noise, quantization noise, image denoising, multiplicative Gaussian noise, comfort noise and lossy compression of noisy images. Communication group includes JPEG transmission errors and JPEG2000 transmission errors. Blur group consists of Gaussian blur and sparse sampling and reconstruction. Color distortions contain change of color saturation, image color quantization with dither and chromatic aberrations. Global distortions include intensity shift and contrast change. Local distortions contain non-eccentricity pattern noise and local block-wise distortions of different intensity. 



\subsection{Performance metrics and compared quality estimators}
\label{subsec:val_metrics}
The performance of the quality estimators are validated using Pearson and Spearman correlation coefficients. Since linearity-based Pearson correlation is sensitive to the range and distribution of the scores, monotonic regression is used before the correlation calculation given in \cite{live2006}.

In the performance comparison, we use fidelity, perceptually-extended fidelity, different types of structural, feature and perceptual similarity-based full reference quality estimators, that include PSNR, PSNR-HA, PSNR-HMA, SSIM, MS-SSIM, CW-SSIM, IW-SSIM, SR-SSIM, FSIMc and PerSIM.



\begin{center}
\input{tab_results_all}
\end{center}




\begin{center}
\input{fig_scatter.tex}
\end{center}

\vspace{-5.0mm}

\subsection{Results}
\label{subsec:val_results}
Performance of the quality estimators in overall databases is summarized in Table \ref{tab_results_databases} and highest two performance results are highlighted with bold in each category. \texttt{UNIQUE} is the best performing quality estimator in TID13 database. In MULTI, \texttt{UNIQUE} is the second highest performing method after SR-SIM in terms of Pearson and after IW-SSIM along with SR-SIM and FSIMc in Spearman. In LIVE, \texttt{UNIQUE} is the second highest performing method after PSNR-HMA in terms of Pearson and it follows IW-SSIM, FSIMc and SR-SIM in terms of Spearman. \texttt{UNIQUE} is not directly compared with other data-driven methods because they usually require database-specific training but most of the reported results in the literature \cite{Ye2012,Ye2013,Gu2014,liu2008,chang2012} are lower than \texttt{UNIQUE}'s results.  

In order to analyze the distribution of subjective scores versus objective quality estimates, scatter plots of the best performing methods are given in Fig. \ref{fig:Scatter}. In the LIVE database, estimated quality scores of IW-SSIM and SR-SIM are mostly located around the high quality region and they follow a monotonically decreasing pattern, whose decrease is very sharp close to the quality score corresponding to the distortion-free images. The average behavior of the FSIMc scores follow a slightly parabolic behavior, where the estimated scores slightly increase and then decrease. PSNR-HMA follows a slightly monotonic behavior and uses most of the quality score range. PerSIM and \texttt{UNIQUE} are the only quality estimators whose scores follow an almost linear behavior all over the quality range. 

In the TID database, SR-SIM and FSIMc use less than half of the quality range with a monotonically increasing behavior. IW-SSIM distribution behaves similarly but uses a slightly wider range. PSNR-HMA follows a parabolic behavior using three quarters of the score range. PerSIM and \texttt{UNIQUE} still use the full quality range with almost linear behavior. 

In MULTI, PerSIM is the only quality estimator that uses the full quality range with almost linear behavior with a relatively high standard deviation. PSNR-HMA is similar to PerSIM but it uses $60 \%$ of the quality range and most of the scores are located around low scores. SR-SIM is mostly linear other than the very high quality scores and it only uses $12\%$ of the quality range. IW-SSIM, FSIMc and \texttt{UNIQUE} follow a monotonically decreasing behavior and  \texttt{UNIQUE} spans a higher quality range than others. 

Overall, the proposed method \texttt{UNIQUE} uses most of the quality range, follows an almost linear behavior in LIVE and TID13 databases even before linear regression  stage and a monotonic behavior in MULTI database.




==> tab_results.tex <==
\begin{table*}[htbp!]
\scriptsize
\centering
\caption{Performance of IQA methods using 5-fold validation for 2,200 runs }
\label{tab_part1}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
               & \textbf{PSNR} & \textbf{PSNR-HA} & \textbf{PSNR-HMA} & \textbf{SSIM} & \textbf{MS-SSIM} & \textbf{CW-SSIM} & \textbf{IW-SSIM} & \textbf{SR-SIM}  & \textbf{FSIMc} & \textbf{PerSIM} &\bf UNIQUE    \\ \cline{2-12}
         
               & \multicolumn{11}{c|}{\textbf{Root Mean Square Error}}                                                                                                                                                                        \\ \hline
\textbf{LIVE} &8.60    &6.92    &\bf 6.57    &7.52    &7.43   &11.2    &7.11    &7.54    &7.20    &6.80    &6.76    \\ \hline
\textbf{MULTI} &12.7   &11.3   &10.7   &11.0   &11.2   &18.8   &10.0    &8.67   &10.7    &9.90   & \bf 8.36
  \\ \hline

         
         
               & \multicolumn{11}{c|}{\textbf{Pearson Correlation Coefficicent}}                                                                                                                                                                        \\ \hline
\textbf{LIVE}     & 0.927   & 0.953    &\bf 0.958   & 0.945   & 0.946    &0.871   &0.951   & 0.945    &0.950   & 0.955  &  0.955
      \\ \hline
\textbf{MULTI}     & 0.735  &  0.798   & 0.819   & 0.812  &  0.802 &   0.402  &  0.847   & 0.887  &  0.821  &  0.850 & \bf  0.895
    \\ \hline

\textbf{}      & \multicolumn{11}{c|}{\textbf{Spearman Correlation Coefficient}}                                                                                                                                                                        \\ \hline
\textbf{LIVE}    & 0.907 &   0.936 &   0.942 &   0.948 &   0.949  &  0.900 &   \bf 0.958  &  0.954 &   \bf 0.958 &   0.948 &   0.950
    \\ \hline
\textbf{MULTI}   &  0.670   & 0.708 &   0.737  &  0.854 &   0.830 &   0.624  &  \bf 0.878  &  0.861 &   0.861 &   0.812  &  0.861
  
        \\ \hline

\end{tabular}
\end{table*}
